CMAL: A Novel Cross-Modal Associative Learning Framework for Vision-Language Pre-Training

With the flourishing of social media platforms, vision-language pre-training (VLP) recently has received great attention and many remarkable progresses have been achieved. The success of VLP largely benefits from the information complementation and enhancement between different modalities. However, most of recent studies focus on cross-modal contrastive learning (CMCL) to promote image-text alignment by pulling embeddings of positive sample pairs together while pushing those of negative pairs apart, which ignores the natural asymmetry property between different modalities and requires large-scale image-text corpus to achieve arduous progress. To mitigate this predicament, we propose CMAL, a Cross-Modal Associative Learning framework with anchor points detection and cross-modal associative learning for VLP. Specifically, we first respectively embed visual objects and textual tokens into separate hypersphere spaces to learn intra-modal hidden features, and then design a cross-modal associative prompt layer to perform anchor point masking and swap feature filling for constructing a hybrid cross-modal associative prompt. Afterwards, we exploit a unified semantic encoder to learn their cross-modal interactive features for context adaptation. Finally, we design an associative mapping classification layer to learn potential associative mappings between modalities at anchor points, within which we develop a fresh self-supervised associative mapping classification task to boost CMAL's performance. Experimental results verify the effectiveness of CMAL, showing that it achieves competitive performance against previous CMCL-based methods on four common downstream vision-and-language tasks, with significantly fewer corpus. Especially, CMAL obtains new state-of-the-art results on SNLI-VE and REC (testA).

==> Appendices.tex <==
% !TEX spellcheck = en_US
% !TeX root = main.tex

\clearpage

\section{Appendices}
\label{sec:appendix}
\subsection{Hyperparameters Setting}
\label{subsec: hypersetting}
The hyperparameters used for MMD dataset are shown in Table~\ref{tab:hyperparameters}.
\begin{table}[htbp]
	\centering
	\begin{tabular}{l|l}
		\hline
		\textbf{Hyperparameter Name} & \textbf{MMD}  \\
		\hline \hline
		Batch Size & 64     \\
		Epoches & 10,000 \\
		Text Embedding Size & 512   \\
		Image Embedding Size & 512    \\
		Transformer Embedding Size & 512 \\
		Learning Rate & 0.0001  \\
		Dropout Ratio & 0.15   \\
		Teacher Forcing Ratio & 0.9   \\
		Mask Length &  6 \\
		Mask Probability  &  0.15 \\
		Replace Probability & 0.15 \\
		Vocabulary Size & 26,422 \\
		\hline
	\end{tabular}%
	\caption{Hyperparameters we used for MMD.}
	\label{tab:hyperparameters}
	\vspace{-1em}
\end{table}%

\subsection{Description of Special Tokens}
The special tokens used in our experiments are shown in Table~\ref{tab:special_token}.

\subsection{Loss Function}
Our total loss function $\mathcal{L}_{Total}$ comprises three parts: UTS encoder loss $\mathcal{L}_{E}$, FAIR layer loss $\mathcal{L}_{F}$ and HTR decoder loss $\mathcal{L}_{D}$, which can be calculated as follows:
\begin{equation}
	\mathcal{L}_{Total}=\gamma_{E} \mathcal{L}_{E}+\gamma_{F} \mathcal{L}_{F}+\gamma_{D} \mathcal{L}_{D}
\end{equation}
where $\gamma_{E}$, $\gamma_{F}$ and $\gamma_{D}$ are hyperparameters, and are initialized equally, i.e., $0.33$, $0.33$ and $0.33$. Then, we tune them on the verification set to obtain a better weight setting of $0.30$, $0.35$ and $0.35$.

The UTS encoder loss $\mathcal{L}_{E}$ contains two parts: $\mathcal{L}_{\mathrm{MLM}}$ and $\mathcal{L}_{\mathrm{MPM}}$,
\begin{equation}
	\mathcal{L}_{E}=\mathcal{L}_{\mathrm{MLM}}+\mathcal{L}_{\mathrm{MPM}}
\end{equation}
the FAIR layer loss contains three parts: $\mathcal{L}_{\mathrm{ITM}}$, $\mathcal{L}_{\mathrm{WPA}}$ and $\mathcal{L}_{\mathrm{IC}}$:
\begin{equation}
	\mathcal{L}_{F}=\mathcal{L}_{\mathrm{ITM}}+\mathcal{L}_{\mathrm{WPA}}+\mathcal{L}_{\mathrm{IC}}
\end{equation}
and the HTR decoder loss is divided into two types: the textual decoding loss $\mathcal{L}_{\mathrm{TXT}}$ for text task and image recommend loss $\mathcal{L}_{\mathrm{IMG}}$ for image task, which is consistent with previous work~\cite{DBLP:conf/mm/NieWHWT19}.  
\begin{equation}
	\mathcal{L}_{D}=\mathcal{L}_{\mathrm{TXT}}+\mathcal{L}_{\mathrm{IMG}}
\end{equation}

\begin{table}[]
	\centering
	\begin{tabular}{l|l}
		\hline
		\textbf{Token}      & \textbf{Description}                    \\ \hline \hline
		{[}CLS{]}  & Utterances classfication token \\ \hline
		{[}TXT{]}  & Text token                     \\ \hline
		{[}IMG{]}  & Image token                    \\ \hline
		{[}KNG{]}  & Knowledge token                \\ \hline
		{[}MASK{]} & Mask token                     \\ \hline
		{[}URL{]} & Image link token  \\ \hline
		{[}PAD{]} & Padding token  \\ \hline
		{[}UNK{]} & Unknown token  \\ \hline
	\end{tabular}
	\caption{Description of special tokens in our experiments.}
	\label{tab:special_token}
	\vspace{-1em}
\end{table}

\subsection{Dateset Statistics}
\label{sec: statistics}
A detailed statistics of the MMD dataset is presented in Table~\ref{tab: detail_statistics}.
\begin{table}[]
	\centering
	\begin{tabular}{l|c|c|c}
		\hline
		\textbf{Dataset Statistics}                       & \textbf{Train}   & \textbf{Valid}  & \textbf{Test}   \\ \hline \hline
		Dialogs             & 105,439 & 22,595 & 22,595 \\ \hline
		Proportion           & 70\%    & 15\%   & 15\%   \\ \hline
		Questions      & 2M      & 446K   & 445K   \\  \hline
		Image Responses         & 904K    & 194K   & 193K   \\  \hline
		Text Responses          & 1.54M   & 331K   & 330K   \\  \hline
		Avg. Utterances            & 40      & 40     & 40     \\  \hline
		Avg. Pos. Images  & 4       & 4      & 4      \\  \hline
		Avg. Neg. Images & 4       & 4      & 4      \\  \hline
		Avg. Words in Question       & 12      & 12     & 12     \\  \hline
		Avg. Words in Response            & 14      & 14     & 14     \\ \hline
	\end{tabular}
	\caption{Detailed statistics of the MMD dataset.}
	\label{tab: detail_statistics}
	\vspace{-1em}
\end{table}

\subsection{Error Analysis}
To better understand the limitations of our model, we conduct an error analysis on UniTranSeR. We randomly select $100$ responses generated by UniTranSeR that achieve low human evaluation scores in the test set of MMD. We report several reasons for the low  scores, which can roughly be classified into four categories. (1) KB information in the generated responses is incorrect ($38\%$), especially when the corresponding equipped knowledge base is large and complex. (2) The sentence structure of the generated responses is incorrect and there are serious grammatical and semantic errors ($24\%$). (3) The model makes incomplete response when there are multiple intentions contained in users' utterances ($21\%$). 
(4) The model selects incorrect product images since different products have similar attributes ($17\%$).

==> results.tex <==
% !TEX spellcheck = en_US
% !TeX root = main.tex

\subsection{Response Quality Evaluation}
%We first evaluate the response quality of IR-Net automatically and manually.



 



\setlength{\tabcolsep}{2.2pt}
\begin{table}[]
	\small
	\centering
	\begin{tabular}{l|c|c|c|c|c|c}
		\hline
		\textbf{Model} &
		\textbf{Flue.} &
		\textbf{Rele.} &
		\textbf{Corr.} &
		\textbf{Info.} &
		\begin{tabular}[c]{@{}l@{}}\textbf{Overall}\\ \textbf{Average}\end{tabular} &
		\begin{tabular}[c]{@{}l@{}}\textbf{Achieve}\\ \textbf{Ratio}\end{tabular} \\ \hline\hline
		\textbf{UMD}        & 2.25 & 2.84 & 3.20 & 2.20 & 2.62 & 54.1\% \\
		\textbf{OAM}        & 2.45 & 2.90 & 3.38 & 3.10 & 2.96 & 61.2\% \\
		\textbf{MAGIC}      & 2.20 & 3.15 & 3.45 & 3.88 & 3.17 & 65.5\% \\
		\textbf{MATE}       & 3.24 & 3.08 & 3.56 & 4.12 & 3.50 & 72.3\% \\ \hline\hline
		\textbf{UniTranSeR} & \textbf{3.65} & \textbf{4.00} & \textbf{3.92} & \textbf{4.22} & \textbf{3.95} & \textbf{81.6\%} \\ \hline
		\textbf{Golden}     & 4.95 & 4.82 & 4.85 & 4.75 & 4.84 & 100\%  \\ \hline
	\end{tabular}
	\vspace{-1em}
	\caption{Human evaluation of responses on fluency (Flue.), relevance (Rele.), correctness (Corr.), informativeness (Info.) on randomly selected dialogs.}
	\label{table: human}
	\vspace{-1em}
\end{table}


%Both automatic and human evaluations indicate the effectiveness of UniTranSeR in terms of the overall generated responses, and the next experiment will evaluate its effectiveness in terms of the individual components of the model.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\subsection{Ablation Study}
In this part, we perform ablation experiments to evaluate the effectiveness of each component. We focus on five crucial components and set them accordingly: 1) w/o UTS Encoder denotes that we use a BiGRU to replace the unified-modal Transformer encoder for multimodal encoding;  
2) w/o HTR Decoder denotes that we use a Uni-directional GRU to replace the hierarchical Transformer decoder for response generation; 3) w/o ITM denotes that we remove the $\mathcal{L}_{\mathrm{ITM}}$ loss to make the parameters not updated; 4) w/o WPA denotes that we remove the $\mathcal{L}_{\mathrm{WPA}}$ loss and just regard the sentence-level representation $f($[CLS]$)$ as query vector $\mathbf{Q}$ to query knowledge; 5) w/o IR Module denotes that we remove the IC and KQ components and just adopt the context vector $f($[CLS]$)$ to generate responses\footnote{Equivalent to generating general responses, since there is no knowledge query.}; 
From Table~\ref{table: ablation}, we can observe that removing each component will result in a performance degradation. Specifically, w/o IR Module causes 54.96\% drops in Bleu-4 score and 54.18\% drops in Nist score, which verifies the great efficacy of intention classify and knowledge query components. Moreover, w/o WPA, w/o ITM and w/o UTS Encoder respectively cause 28.54\%, 20.48\% and 14.37\% drops in Nist score, which further demonstrates the effectiveness of cross-modal feature alignment and unified-modal semantic encoding. 

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{img/case.pdf}
	\caption{Visualization of Feature Alignment.}
	\label{fig: case}
	\vspace{-1em}
\end{figure}


\subsection{Case Study and Visualization}
To better illustrate the advantage of our model and understand what the feature alignment module has learned, we visualize several examples of text-to-image attention, as shown in Figure~\ref{fig: case}. It can be observed that our model is able to capture fine-grained entity alignment between different modalities. The reason may be that: 1) We adopt a unified-modal Transformer semantic encoder, which enables to map different modalities of semantic cues into a same vector space to prompt inter-modality interactions for better representations; 2) Based on the obtained representations, the WPA technology can help supervise fine-grained word-patch alignment, which is beneficial to identifying user's real intention and generate more intention-aware responses.
%while previous multimodal dialog model, which is limited in capturing the fine-grained alignment, since there is no projecting the multimodal semantic features into a unified vector space and training them to prompt cross-modality entity alignment. 




\setlength{\tabcolsep}{2pt}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 









